Guidance Free Image Editing via Explicit Conditioning

Current sampling mechanisms for conditional diffusion models rely mainly on Classifier Free Guidance (CFG) to generate high-quality images. However, CFG requires several denoising passes in each time step, e.g., up to three passes in image editing tasks, resulting in excessive computational costs. This paper introduces a novel conditioning technique to ease the computational burden of the well-established guidance techniques, thereby significantly improving the inference time of diffusion models. We present Explicit Conditioning (EC) of the noise distribution on the input modalities to achieve this. Intuitively, we model the noise to guide the conditional diffusion model during the diffusion process. We present evaluations on image editing tasks and demonstrate that EC outperforms CFG in generating diverse high-quality images with significantly reduced computations.

==> figs/conditioning/figure.tex <==
\begin{figure*}
\label{fig:method}
\centering
%\begin{overpic}[width=\textwidth]{figs/conditioning/conditioning} % add grid to the paramters to see the grid
%    \centering
%    \put(120,43){$\mu^I_\psi$}
%    \put(120,23){$\Sigma^I_\psi$}
%    \put(192,75){$\mu^P_\psi$}
%    \put(211,75){$\Sigma^P_\psi$}
%\end{overpic}
\includegraphics[width=\textwidth]{figs/conditioning/conditioning}

\caption{We encode the image into a normal distribution $\mathcal{N}(\mu^I_\psi(c_I),\Sigma^I_\psi(c_I)*\mathbf{I})$. We use a clip encoder~\cite{Radford_2021} to obtain embeddings from a text prompt. A variational text encoder maps the pooled embeddings $\bar{p}$ to a latent distribution $\mathcal{N}(\mu^P_\psi(c_P),\Sigma^P_\psi(c_P)*\mathbf{I})$. These distributions are merged together to model the noise. We sample from the joint distribution a noise vector and denoise it through a UNet. Finally, we decode the denoised latent into an image.}

\end{figure*}

